Fast Object Detection with Latticed Multi-Scale Feature Fusion

Scale variance is one of the crucial challenges in multi-scale object detection. Early approaches address this problem by exploiting the image and feature pyramid, which raises suboptimal results with computation burden and constrains from inherent network structures. Pioneering works also propose multi-scale (i.e., multi-level and multi-branch) feature fusions to remedy the issue and have achieved encouraging progress. However, existing fusions still have certain limitations such as feature scale inconsistency, ignorance of level-wise semantic transformation, and coarse granularity. In this work, we present a novel module, the Fluff block, to alleviate drawbacks of current multi-scale fusion methods and facilitate multi-scale object detection. Specifically, Fluff leverages both multi-level and multi-branch schemes with dilated convolutions to have rapid, effective and finer-grained feature fusions. Furthermore, we integrate Fluff to SSD as FluffNet, a powerful real-time single-stage detector for multi-scale object detection. Empirical results on MS COCO and PASCAL VOC have demonstrated that FluffNet obtains remarkable efficiency with state-of-the-art accuracy. Additionally, we indicate the great generality of the Fluff block by showing how to embed it to other widely-used detectors as well.

==> README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

IEEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************


==> exp-discussion.tex <==
%PASCAL VOC has played an important role in promoting early object detection. However, its current space for improvement is relatively limited, and the transfer bar of the authoritative evaluation set is gradually passed to MS COCO.
Compared to PASCAL VOC, MS COCO contains more instances per category, and the distribution is more balanced. This dataset also contains more small objects. In addition, MS COCO’s evaluation criteria are more comprehensive than Pascal VOC.
%So in this paper, we mainly focus on the performances of models on MS COCO.
A comparison of some detectors on the MS COCO is shown in Table ~\ref{tab:coco_performance_comparison} . It can be seen that our {\ournet} is the most accurate of the real-time detectors.
%At the same time, our {\ournet}512 not only achieves considerable detection accuracy (mAP) , but also maintains a real-time detection speed of 32FPS.
%As shown in Table ~\ref{tab:voc_performance_comparison}, on the PASCAL VOC, our {\ournet}512 can run at an ultra-high speed of 55.6 FPS and maintain a remarkable accuracy (mAP) of 82.5\%.

As shown in Figure \ref{fig:map-time}, like the M2Det, we plotted the speed-accuracy trade-off curve. Thanks to the one-stage lightweight framework and the {\ourmethod} block, our {\ournet} is able to draw a better speed-accuracy curve than other detectors (\ie as shown in the figure,  the curve of  {\ournet}  is located at the top left of all detectors, meaning that our detector outperforms other detectors in terms of speed-accuracy synthesis).
This is because we have designed a multi-level and multi-scale fine-grained feature fusion module, {\ourmethod}, for two problems existed in the multi-scale feature fusion method in the current object detection domain.
The {\ourmethod} block can achieve further fine-grained fusion of the detailed features in the network based on the current feature fusion methods. And by applying the {\ourmethod} block to the one-stage lightweight network, SSD~\cite{liu2016ssd}, we designed {\ournet} to greatly improve the detection accuracy while ensuring the extremely high detection speed of the lightweight network. 

==> exp-not-work-design.tex <==
\subsubsection{Use con3x3 to change the channel of feature}
As shown in Figure 1, when the feature enters the block, it needs to be convolved to change channels of the feature map. Inspired by RFBNet, we tried to use conv3x3 to change the number of feature's channels. However, its map is 1\% lower than conv1x1 and 3ms slower.
\subsubsection{Apply the Se-attention to the block}
In the block, the features generated by different branches of each layer of the block are combined by the Concat function. We tried the Se-attention mechanism and weighted the various channels of the Features, but did not achieve the desired effect. 

==> method-alg.tex <==
\begin{table}[ht]
\begin{tabular}{lp{2cm}}
\hline
\textbf{ Algorithm 1}: The process of {\ourmethod}  block operation\\
\hline
\textbf{input}:PreVious Features: $X_p$,size is $[b,h_{in},w_{in},c_{in}]$.\\
\textbf{output}:Out Features: $X_{out}$,size is $[b,h_{o},w_{o},c_{o}]$.\\
\\
\textbf{Step 1}: Define $c_{inter} = c_{in}//8$; Scale and \\
channel transform is performed on input feature $X_p$ \\
through Conv1x1, get $X_{in}$, and the size of $X_{in}$ \\
is $[b,h_o,w_o,2*c_{inter}]$. $X_{in}$ is passed through the \\
multi-branch structure of the first layer to generate \\
features of four different scale receptive fields,\\
which are named $X_{00}, X_{01}, X_{02}, X_{03}$.\\
After being activated by the Relu function, \\
$X_{0j\_r} = Relu(X_{0j}) (j=0, 1, 2, 3)$ is obtained.\\
\\
\textbf{Step 2}: Input $X_{0j} (j=0,1,2,3)$ into the second\\
layer to get $X_{1j}(j=0,1,2,3)$. After activation by Relu \\
function, we get $X_{1j\_r} = Relu(X_{1j})(j=0,1,2,3)$.Similarly,\\
let $X_{1j\_r}$ passes through the third layer to get \\
$X_{2j} (j=0,1,2,3)$.\\
\\
\textbf{Step 3}: Let $X_c = Concat(X_{ij})(i=0,1,2;j=0,1,2,3)$ \\
(size is $[b,h_o,w_o,24*c_{inter}]$),\\
define$X_{shortcut}=shortCut(X_p)$(size is \\
$[b,h_o,w_o,c_o]$), convert the number of channels of $X_c$ \\
by Conv1x1, and get $X_{c\_o}$, whose size is $[b,h_o,w_o,c_o]$. \\
Then get the out feature : $X_{out} = X_{c\_o} + X_{shortcut}$.\\
\hline
\end{tabular}
\end{table}


==> test.tex <==
Our fine-grained feature fusion module mainly acts on local features in the network. Most of the traditional feature fusion modules will act on the global features generated in the whole network, and achieve coarse-grained feature fusion of multi-scale features generated by multiple layers in the network.In other words, the module will work simultaneously on multiple feature maps in the network. However,our block will only work for a certain size feature at a time, that is, our block will only act on local features in the network, rather than acting on the entire network as in traditional feature fusion operations. 
